Structured Low-Rank Tensors for Generalized Linear Models

Recent works have shown that imposing tensor structures on the coefficient tensor in regression problems can lead to more reliable parameter estimation and lower sample complexity compared to vector-based methods. This work investigates a new low-rank tensor model, called Low Separation Rank (LSR), in Generalized Linear Model (GLM) problems. The LSR model -- which generalizes the well-known Tucker and CANDECOMP/PARAFAC (CP) models, and is a special case of the Block Tensor Decomposition (BTD) model -- is imposed onto the coefficient tensor in the GLM model. This work proposes a block coordinate descent algorithm for parameter estimation in LSR-structured tensor GLMs. Most importantly, it derives a minimax lower bound on the error threshold on estimating the coefficient tensor in LSR tensor GLM problems. The minimax bound is proportional to the intrinsic degrees of freedom in the LSR tensor GLM problem, suggesting that its sample complexity may be significantly lower than that of vectorized GLMs. This result can also be specialised to lower bound the estimation error in CP and Tucker-structured GLMs. The derived bounds are comparable to tight bounds in the literature for Tucker linear regression, and the tightness of the minimax lower bound is further assessed numerically. Finally, numerical experiments on synthetic datasets demonstrate the efficacy of the proposed LSR tensor model for three regression types (linear, logistic and Poisson). Experiments on a collection of medical imaging datasets demonstrate the usefulness of the LSR model over other tensor models (Tucker and CP) on real, imbalanced data with limited available samples.

==> Conclusion.tex <==
In this work, we proposed a new tensor structure for parameter estimation in regression problems. Specifically, we imposed a low-rank LSR tensor structure on the coefficient tensor for GLMs. 
We formulated the parameter estimation problem and proposed a block coordinate descent algorithm to estimate the coefficient tensor under the LSR model. We investigated the effectiveness of our proposed approach on synthetic data and several significant biological imaging data. Our theoretical guarantees include deriving minimax lower bounds on the estimation error of the LSR structured coefficient tensor. We empirically assess the tightness of the bound for several regression types. 
 
